Improved Approximation Algorithms for (1,2)-TSP and Max-TSP Using Path Covers in the Semi-Streaming Model

We investigate semi-streaming algorithms for the Traveling Salesman Problem (TSP). Specifically, we focus on a variant known as the $(1,2)$-TSP, where the distances between any two vertices are either one or two. Our primary emphasis is on the closely related Maximum Path Cover Problem, which aims to find a collection of vertex-disjoint paths that cover the maximum number of edges in a graph. We propose an algorithm that, for any $\epsilon > 0$, achieves a $(\frac{2}{3}-\epsilon)$-approximation of the maximum path cover size for an $n$-vertex graph, using $\text{poly}(\frac{1}{\epsilon})$ passes. This result improves upon the previous $\frac{1}{2}$-approximation by Behnezhad et al. [ICALP 2024] in the semi-streaming model. Building on this result, we design a semi-streaming algorithm that constructs a tour for an instance of $(1,2)$-TSP with an approximation factor of $(\frac{4}{3} + \epsilon)$, improving upon the previous $\frac{3}{2}$-approximation actor algorithm by Behnezhad et al. [ICALP 2024] (Although it is not explicitly stated in the paper that their algorithm works in the semi-streaming model, it is easy to verify). Furthermore, we extend our approach to develop an approximation algorithm for the Maximum TSP (Max-TSP), where the goal is to find a Hamiltonian cycle with the maximum possible weight in a given weighted graph $G$. Our algorithm provides a $(\frac{7}{12} - \epsilon)$-approximation for Max-TSP in $\text{poly}(\frac{1}{\epsilon})$ passes, improving on the previously known $(\frac{1}{2}-\epsilon)$-approximation obtained via maximum weight matching in the semi-streaming model.

==> MPC/CorrectnessMPC.tex <==
%\subsection{Correctness of \hyperref[alg1]{Algorithm 1}}








==> MPC/Proof-Lemma-3.5.tex <==

\section{Proof of \hyperref[correct-alg1]{Lemma \ref*{correct-alg1}}}\label{appendix-lemma-3.5}



We claim that $M_1 \cup M_2$ is a vertex-disjoint union of paths of length $1,2$ or $3$. As a result, it is a path cover. Suppose $ M_1 = \{ u_1v_1, u_2v_2, \ldots , u_kv_k \}$. Let us denote the vertices of $ G/ M_1$ by
$ \{ (uv)_1, (uv)_2, \ldots , (uv)_k, w_1,w_2,\ldots, w_l \} $ where $(uv)_i$ represents the vertices $u_i$ and $v_i$, merged in the contracted graph $G/M_1$ and $w_j$'s for $1 \leq j \leq l$ are the rest of the vertices. Let $xy \in M_2$ be an arbitrary edge. By symmetry between $x$ and $y$, there are three cases as follows:
\begin{enumerate}
    \item $x,y \in \{w_1, w_2,\ldots, w_l\}$.\\
    In this case, $ x $ and $ y $ are intact vertices after contraction, which means there are no edges in $ M_1 $ adjacent to $x $ and $ y$. Since $xy \in M_2$ and $M_2$ is a matching, there are no other edges in $ M_1 \cup M_2 $ adjacent to $ x $ and $ y $ in $ G $. As a result, $xy$ would be a path of length $1$ in $M_1 \cup M_2$.
    \item $ x \in \{ (uv)_1, (uv)_2, \ldots , (uv)_k \} $ and $ y \in \{w_1, w_2,\ldots, w_l\}$.\\
    In this case, $ x= (uv)_i $ for some $ 1 \leq i \leq k$. As a result, $ xy $ would be $ u_iy $ or $ v_iy $ in $ G $. By symmetry, assume that $xy=u_iy$ in $G$. Since $M_1$ is a matching, no other edges in $M_1$ are adjacent to $u_i$ and $v_i$. No edge in $M_1$ is adjacent to $y$. Since $M_2$ is a matching, the only edge in $M_2$ adjacent to at least one of $u_i,v_i$ and $y$ in $G$ is $xy=u_iy$. Finally, we can see that $(v_i,u_i,y)$ is a path of length $2$ in $M_1 \cup M_2$.
    \item $x,y \in \{ (uv)_1, (uv)_2, \ldots , (uv)_k \}$.\\
    In this case, let $ x=(uv)_i$ and $y=(uv)_j$ and by symmetry, assume that $xy$ is the edge connecting $u_i$ to $u_j$ in $ G $. Since $M_1$ is a matching, the only edges in $M_1$ adjacent to at least one of $u_i,u_j,v_i,v_j$ are $u_iv_i$ and $u_jv_j$. Since $M_2$ is a matching, the only edge in $M_2$ adjacent to at least one of $u_i,u_j,v_i,v_j$ is $(uv)_i(uv)_j$. As a result, $(v_i,u_i,u_j,v_j)$ would be a path of length $3$ in $M_1 \cup M_2$.
\end{enumerate}
So, $M_1 \cup M_2$ is a union of vertex-disjoint paths of length $1,2$ or $3$.
